If at First You Don't Succeed, Try, Try Again: Faithful Diffusion-based Text-to-Image Generation by Selection

Despite their impressive capabilities, diffusion-based text-to-image (T2I) models can lack faithfulness to the text prompt, where generated images may not contain all the mentioned objects, attributes or relations. To alleviate these issues, recent works proposed post-hoc methods to improve model faithfulness without costly retraining, by modifying how the model utilizes the input prompt. In this work, we take a step back and show that large T2I diffusion models are more faithful than usually assumed, and can generate images faithful to even complex prompts without the need to manipulate the generative process. Based on that, we show how faithfulness can be simply treated as a candidate selection problem instead, and introduce a straightforward pipeline that generates candidate images for a text prompt and picks the best one according to an automatic scoring system that can leverage already existing T2I evaluation metrics. Quantitative comparisons alongside user studies on diverse benchmarks show consistently improved faithfulness over post-hoc enhancement methods, with comparable or lower computational cost. Code is available at \url{https://github.com/ExplainableML/ImageSelect}.

==> tables/full_diverse_prompts.tex <==
\begin{table}[t]
    \centering
    \caption{Summary of the prompt distribution and their origin in the full set of \texttt{diverse}-prompt collections.}    
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
    \toprule
         \textbf{Dataset} & \texttt{diverse-1k} & \texttt{diverse-2k} & \texttt{diverse-4k} & \texttt{diverse-8k} & \texttt{diverse-16k}\\
         \midrule
        HRS (Bias) \cite{hrs} &  38 & 76 & 151 & 331 & 986 \\
        HRS (Color) \cite{hrs} &  38 & 76 & 151 & 316 & 468 \\
        HRS (Counting) \cite{hrs} &  38 & 76 & 153 & 333 & 1097 \\
        HRS (Emotion) \cite{hrs} &  38 & 76 & 153 & 333 & 1099 \\
        HRS (Fair Styles) \cite{hrs} &  38 & 76 & 153 & 216 & 216 \\
        HRS (Long) \cite{hrs} &  38 & 76 & 151 & 319 & 873 \\
        HRS (Size) \cite{hrs} &  38 & 74 & 147 & 259 & 361 \\
        HRS (Spatial) \cite{hrs} &  38 & 72 & 143 & 311 & 807 \\
        HRS (Long Synthetic) \cite{hrs} &  38 & 76 & 151 & 319 & 1009 \\
        HRS (Writing) \cite{hrs} &  36 & 72 & 148 & 305 & 938 \\
        Struct. Diff. (ABC) \cite{feng2023structured} &  127 & 254 & 508 & 1100 & 3572 \\
        Struct. Diff. (CC) \cite{feng2023structured} &  125 & 243 & 478 & 551 & 548 \\
        TIFA \cite{hu2023tifa} &  381 & 759 & 1518 & 3309 & 4026 \\
        \midrule
        \textbf{Total} & 1011 & 2006 & 4005 & 8002 & 16000 \\
    \bottomrule
    \end{tabular}}
    \label{tab:diverse_prompts}
\end{table}

==> tables/quantiative.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
Model                   & TIFA Score & ImageReward \\ 
\midrule
Stable Diffusion 1.4 \cite{rombach22ldm} & 0.72     & -0.22       \\
Composable Diffusion \cite{compt2i} & 0.72     & -0.35      \\
Structure Diffusion \cite{feng2023structured} & 0.71     & -0.35      \\
Attend-and-Excite++ (ours, 1.4) \cite{chefer2023attendandexcite} & 0.75     & 0.04       \\
ImageReward-Selection (ours)  & \textbf{0.81}     & N/A      \\
TIFA-Selection (ours)         & N/A     & \textbf{0.32}       \\
\midrule
Stable Diffusion 2.1 \cite{rombach22ldm} & 0.76     & 0.19       \\
Attend-and-Excite++ (ours, 2.1) \cite{chefer2023attendandexcite} & 0.78     & 0.36       \\
Image-Reward-Selection (ours) & \textbf{0.83}     & N/A       \\
TIFA-Selection (ours) & N/A     & \textbf{0.59}      \\ 
\bottomrule
\end{tabular}
\caption{Results on \benchmarkName  showing that selecting the best image from a pool of 10 random generations significantly outperforms both the base Stable Diffusion, and other post-hoc enhancement methods on the TIFA and ImageReward metrics.}
\end{table}


==> tables/userstudy.tex <==
\begin{table}[]
\begin{tabular}{ll}
\hline
Model                   & Win Rate \\ \hline
Structure Diffusion     & 68.62\%   \\
Composable Diffusion    & 74.53\%   \\
Attend-and-Excite (1.4) & 68.02\%   \\ \midrule
Attend-and-Excite (2.1) & 66.66\%   \\ \bottomrule
\end{tabular}
\caption{Results of our User Study}
\label{tab:user}
\end{table}
